Denoising Likelihood Score Matching for Conditional Score-based Data Generation

Many existing conditional score-based data generation methods utilize Bayes' theorem to decompose the gradients of a log posterior density into a mixture of scores. These methods facilitate the training procedure of conditional score models, as a mixture of scores can be separately estimated using a score model and a classifier. However, our analysis indicates that the training objectives for the classifier in these methods may lead to a serious score mismatch issue, which corresponds to the situation that the estimated scores deviate from the true ones. Such an issue causes the samples to be misled by the deviated scores during the diffusion process, resulting in a degraded sampling quality. To resolve it, we formulate a novel training objective, called Denoising Likelihood Score Matching (DLSM) loss, for the classifier to match the gradients of the true log likelihood density. Our experimental evidence shows that the proposed method outperforms the previous methods on both Cifar-10 and Cifar-100 benchmarks noticeably in terms of several key evaluation metrics. We thus conclude that, by adopting DLSM, the conditional scores can be accurately modeled, and the effect of the score mismatch issue is alleviated.

==> figures/combined_ablation.tex <==
\begin{table}
    \begin{minipage}{0.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/images/curve.pdf}
		\vspace{-2em}
		\captionof{figure}{The curve of the fisher divergence and cross entropy}
		\label{fig:curve}
	\end{minipage}\hfill
	\begin{minipage}{0.45\linewidth}
		\renewcommand{\arraystretch}{1.05}
        \newcommand{\boldtoprule}{\toprule[1.2pt]}
        \centering
        \footnotesize
        \caption{The experimental results with different value of $\lambda$.}
        %\vspace{-1em}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{ccccc}
            \boldtoprule
                         & $\lambda=0.5$ &  $\lambda=1.0$ &  $\lambda=2.0$ & $\lambda=8.0$ \\ 
             \hline
            FID          &  2.33  &  2.25  &  2.36  &  2.25  \\
            IS           &  9.90  &  9.90  &  9.98  &  9.79  \\
            \hline
            Precision    &  0.64  &  0.65  &  0.64  &  0.64  \\
            Recall       &  0.62  &  0.62  &  0.62  &  0.62  \\
            Density      &  0.94  &  0.96  &  0.95  &  0.94  \\
            Coverage     &  0.79  &  0.81  &  0.79  &  0.78  \\
            \boldtoprule
        \end{tabular}}
        \label{tab:lambda}
	\end{minipage}
\end{table}

% \input{figures/curve.tex}
% \input{tables/lambda.tex}

==> tables/benchmark.tex <==
\begin{table}[t]
    \renewcommand{\arraystretch}{1.1}
    \newcommand{\boldtoprule}{\toprule[1.2pt]}
    \centering
    \footnotesize
    \caption{The evaluation results on the Cifar-10 and Cifar-100 benchmarks.}
    %\vspace{-0.5em}
    %\resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|ccc||ccc}
        \boldtoprule
                          && \multicolumn{3}{c||}{Cifar-10}  &  \multicolumn{3}{c}{Cifar-100} \\ 
        %\hline
                          &&  Standard &  Scaled  &  Ours  &  Standard &  Scaled  &  Ours \\ 
        \hline
        FID        & $\downarrow$ &  4.10     &  12.48   &  \textbf{2.25}  &  4.52  & 12.58  &  \textbf{3.86}  \\
        IS         & $\uparrow$   &  9.08     &  9.37    &  \textbf{9.90}  &  11.53 & 11.59 &  \textbf{11.62} \\
        \hline
        Precision   & $\uparrow$ &  0.67     &  \textbf{0.75}    &  0.65  &  0.62     &  \textbf{0.65}    &  0.61  \\
        Recall      & $\uparrow$ &  0.61     &  0.49    &  \textbf{0.62}  &  0.62     &   0.52  &  \textbf{0.63}  \\
        Density     & $\uparrow$ &  1.05     &  \textbf{1.36}    &  0.96  &  0.84     &  \textbf{0.93}    &  0.82  \\
        Coverage    & $\uparrow$ &  0.80     &  0.75    &  \textbf{0.81}  &  \textbf{0.71}     &  0.61  &  \textbf{0.71}  \\
        \hline
        CAS         & $\uparrow$ &  0.38    &   0.46    &  \textbf{0.58}  & 0.15  &  0.24 &  \textbf{0.28}   \\
        \hline \hline
        Precision$^\dagger$  & $\uparrow$ &  0.51     &  \textbf{0.70}    &  0.56  &  0.33  &  \textbf{0.59} &  0.42 \\
        Recall$^\dagger$     & $\uparrow$ &  0.59     &  0.42    &  \textbf{0.61}  &  \textbf{0.68}  &  0.41 &  \textbf{0.68} \\
        Density$^\dagger$    & $\uparrow$ &  0.63     &  \textbf{1.23}    &  0.76  &  0.30  &  \textbf{0.78} &  0.43 \\
        Coverage$^\dagger$   & $\uparrow$ &  0.60     &  0.66    &  \textbf{0.71}  &  0.38  &  0.51 &  \textbf{0.52} \\
        \boldtoprule
    \end{tabular}%}
    \label{tab:benchmark}
\end{table}


==> tables/symbols-old.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.1}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\begin{tabular}{l|l}
\mytoprule
    Symbol & Description  \\
    \mytoprule
    $\x$ & A sample where $\x \in \Rd$ \\
    $y$ & The label of $\x$ \\
    $\tx$ & A perturbed sample \\
    $\z$ & A noise vector\\
    $\X$ & A set of all $\x$ \\
    $\Y$ & A set of all $y$\\
    \hline
    $\D=\{(\x^{(1)},y^{(1)}),...,(\x^{(m)},y^{(m)})\}$ & Training set: i.i.d. samples\\
    $\pd(\x)$ & The unknown true pdf., where $\x \in \Rd$ \\
    $\p(\x)$ & The estimated pdf. of $\x$ \\
    $\q(\tx)$ & The unknown perturbed pdf., where $\tx \in \Rd$\\
    $\q(\tx|\x)$ & Smoothing kernel: isotropic Gaussian of variance $\sigma^2$\\
    $\q(\tx,\x)=\q(\tx|\x) \q(\x)$ & Joint pdf.\\
    $\q(\tx)=\int_x \q(\tx|\x) \q(\x) d\x$ & Parzen density estimate based on $\x\in\D$ obtainable by marginalizing $\q(\tx,\x)$\\
    \hline
    $\langle \mathbf{u},\mathbf{v}\rangle=\sum_i\mathbf{u}_i \mathbf{v}_i $ & Dot product between two vectors \\
    $\| \mathbf{u} \|=\sqrt{\langle \mathbf{u},\mathbf{u}\rangle}$ & Euclidean norm of vector\\
    \mytoprule
\end{tabular}%}
\vspace{0.1ex}
\caption{List of commonly-used symbols.}
\label{tab:notation}
\end{table*}
